$uvby-\beta$ photoelectric photometry of the open clusters NGC 6811 and NGC 6830

From $uvby-\beta$ photometry of the open clusters NGC 6811 (75 stars), and NGC 6830 (19 stars) we were able to determine membership of the stars to each cluster, and fix the age and reddening for each. Since several short period stars have recently been found, we have carried out a study of these variables.

==> Tbl6.tex <==
\setcounter{table}{5}%table 6
\tablecols{12}
\tabcaption{Cross ID and membership probabilities of
the open cluster NGC 6811}
\def\ColumnHeaders{
WBD & Luo & Sanders & Becker & Barkhatova & Kharchenko & Prob Sanders & Pkin & Pph & Psp & mbr\\ }
\begin{longtable}{rcccccclllll}%[]\centering - WJH 02 Apr 2009 shouldn't be here - commented
 %% Primera Cabeza
  \toprule
  \ColumnHeaders\\ \midrule
  \endfirsthead

  %% Otras Cabezas
  \tabcaptioncontinued
  \toprule
  \ColumnHeaders\\ \midrule
  \endhead

  %% Pies normales
  \bottomrule
  \endfoot




112 &    & 177 & 51 & 1136 & & 0 & & & & nm\\
122 &    &     & & & & & & & & nm\\
107 &    & 183 & 48 & & & 96 & & & & nm\\
 31 &    & 102 & 15 & 1057 &  & 97 &  &  &  & m\\
489 & 6  & 205 & & 2080 & & 89 & & & & m\\
146 &    & 187 & 42 & 1143 & & 0 & & & & m\\
 68 &    & 110 & 86 & 1065 & 78 & 97 & 0.9272 & 1 & 1 & m\\
 34 &    & 121 & 22 & 1084 &  & 96 &  &  &  & m\\
105 &    & 185 & 47 & 1141 & & 25 & & & & m\\
 85 &    &  94 & 4 & 1041 &  & 95 &  &  &  & m\\
218 &    & 192 & & 1154 & & 92 & & & & m\\
106 &    & 172 & 49 & 1133 & & 97 & & & & m\\
 47 &    & 158 & 35 & 1121 &  & 96 &  &  &  & m\\
 37 & 2  & 136 & 26 & 1104 &  & 96 &  &  &  & m\\
147 &    & 189 & 43 & 1146 & & 97 & & & & m\\
 70 & 3  & 108 & 82 & 1063 & 76 & 96 & 0.9837 & 1 & 1 & m\\
 86 &    &  98 & 5 & 1050 &  & 89 &  &  &  & m\\
 26 &    &  86 & 10 & 1038 & 69 & 97 & 0.4193 & 1 & 1 & m\\
 99 &    & 159 & 29 & 1122 &  & 97 &  &  &  & m\\
 18 & 1  & 97 & 85 & 1049 & 73 & 97 & 0.0016 & 1 & 1 & m\\
115 &    & 149 & 65 & & & 95 & & & & m\\
 16 &    & 103 & 81 & 1059 &  & 90 &  &  &  & m\\
 54 &    & 147 & 68 & 1114 &  & 97 &  &  &  & m\\
113 & 5  & 166 & 60 & 1126 & 98 & 93 & 0.8128 & 1 & 1 & m\\
 92 &    & 115 & 20 & 1071 &  & 0 &  &  &  & m\\
 46 &    & 160 & 36 & 1124 &  & 96 &  &  &  & m\\
 33 & 13 & 113 & 19 & 1066 & 79 & 95 & 0.9765 & 0.9971 & 1 & m\\
114 &    & 146 & 66 & & & 96 & & & & m\\
 49 &    & 165 & 46 & 1125 & 97 & 93 & 0.7504 & 1 & 1 & m\\
  5 &    & 127 & 25 & 1092 & 83 & 93 & 0.9227 & 0.7357 & 1 & m\\
  9 & 16 & 134 & 71 & 1101 & 86 & 88 & 0.9565 & 1 & 1 & m\\
 62 &    & 123 & 77 & 1087 &  & 97 &  &  &  & m\\
139 &    & 131 & & 1096 & & 95 & & & & m\\
 44 & 11 & 157 & 33 & 1120 & 95 & 96 & 0.9137 & 1 & 1 & m\\
 53 & 10 & 135 & 69 & 1105 &  & 94 &  &  &  & m\\
 45 &    & 155 & 34 & 1118 & 94 & 97 & 0.0001 & 0.6244 & 1 & m\\
 78 &    &  72 & 11 & 1023 &  & 95 &  &  &  & m:\\
 39 & 4  & 144 & 30 & 1112 &  & 54 &  &  &  & nm\\
 41 &    & 154 & 28 & 1117 &  & 0 &  &  &  & nm\\
  8 &    &     &  & 1106 &  &  &  &  &  & nm\\
 56 &    & 138 & 67 & 1108 & 89 & 0 & 0.7463 & 0.9707 & 1 & nm\\
 36 &    & 132 &  & 1099 &  & 97 &  &  &  & nm\\
 42 & 14 & 143 & 31 & 1111 &  & 90 &  &  &  & nm\\
  4 & 12 & 119 & 23 & 1077 &  & 95 &  &  &  & nm\\
 51 & 15 & 137 & 70 & 1109 &  & 97 &  &  &  & nm\\
 43 &    & 142 & 32 & 1110 &  & 96 &  &  &  & nm\\
 40 &    &     &  &  &  &  &  &  &  & nm\\
  6 &    &     &  & 1093 &  &  &  &  &  & und\\
  7 &    &     &  & 1102 &  &  &  &  &  & und\\
 10 &    &     &  & 1085 &  &  &  &  &  & und\\
 12 &    &     &  & 1078 &  &  &  &  &  & und\\
 13 &    &     &  & 1082 &  &  &  &  &  & und\\
 14 &    & 114 & 80 & 1067 &  & 0 &  &  &  & und\\
 22 &    &  84 & 18 & 1029 &  & 0 &  &  &  & und\\
 23 & 18 &     & 17 & 1053 &  &  &  &  &  & und\\
 24 &    &  95 & 14 & 1047 & 72 & 97 & 0.8117 & 1 & 1 & und\\
 32 &    & 106 & 16 & 1061 &  & 97 &  &  &  & und\\
 35 &    & 128 &  & 1095 &  & 80 &  &  &  & und\\
 38 &    & 150 & 27 & 1115 &  & 0 &  &  &  & und\\
 57 &    & 129 & 72 & 1097 &  & 79 &  &  &  & und\\
 58 &    & 130 & 73 & 1098 &  & 71 &  &  &  & und\\
 63 &    &     &  &  &  &  &  &  &  & und\\
 64 &    &     &  &  &  &  &  &  &  & und\\
 65 &    & 120 & 78 & 1081 &  & 96 &  &  &  & und\\
 71 &    &  77 & 100 & 1026 & 66 & 97 & 0.5865 & 1 & 1 & und\\
 73 &    &  64 & 101 & 1016 & 61 & 0 & 0.0646 & 1 & 1 & und\\
 74 &    &  74 & 13 &  &  & 0 &  &  &  & und\\
 77 &    &  67 & 12 & 1018 &  & 97 &  &  &  & und\\
 79 &    &  85 & 1 & 1031 & 68 & 0 & 0.4112 & 1 & 1 & und\\
 82 &    &  89 & 3 & 1036 &  & 27 &  &  &  & und\\
 87 &    & 100 & 7 & 1054 &  & 57 &  &  &  & und\\
101 &    & 170 & 38 & 1131 & 87 & 97 & 0.8326 & 1 & 1 & und\\
102 &    & 179 & 40 & 1137 & & 0 & & & & und\\ 118 & &
145 & 64 &1113 & & 0 & & & & und\\
123 &    &     & & 1051 & & & & & & und\\
133 &    &  92 & 2 & 1039 & 71 & 94 & 0.8766 & 1 & 1 & und\\
178 &    &  76 & 99 & 1025 & 65 & 96 & 0.8519 & 0.9999 & 1 & und\\
491 & 7  & 209 & & & & 0 & & & & und\\
v17 &          & & & & & & & & & und\\
\end{longtable}



